Prototyping Next-Generation O-RAN Research Testbeds with SDRs

Open RAN (O-RAN) defines an emerging cellular radio access network (RAN) architecture for future 6G wireless networks, emphasizing openness and intelligence which are considered the foundations of future 6G wireless networks. While the inherent complexity and flexibility of the RAN give rise to many new research problems, progress in developing solutions is hampered due to the lack of end-to-end, fully developed platforms that can help in pursuing use cases in realistic environments. This has motivated the formation of open-source frameworks available to the wireless community. However, the rapid evolution of dedicated platforms and solutions utilizing various software-based technologies often leaves questions regarding the interoperability and interactions between the components in the framework. This article shows how to build a software-defined radio testbed featuring an open-source 5G system that can interact with the near-real-time (near-RT) RAN intelligent controller (RIC) of the O-RAN architecture through standard interfaces. We focus on the O-RAN E2 interface interactions and outline the procedure to enable a RAN system with E2 capabilities. We demonstrate the working of two xApps on the testbed with detailed E2 message exchange procedures and their role in controlling next-generation RANs.

==> include/HWTable.tex <==
\begin{table*}[h!]
\centering
\caption{USRP feature comparison. \hl{Is this table needed?}} 
\footnotesize
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{0.8cm}|p{1.65cm}|p{1.75cm}|p{1.3cm}|p{0.85cm}|p{1.4cm}|p{1.3cm}|p{1cm}|p{0.95cm}|p{0.75cm}|}
\hline
\textbf{USRP Model} &  \textbf{FPGA} &   \textbf{Daughterboards} &  \textbf{Ethernet Interface} &  \textbf{USB 3.0 } &  \textbf{Frequency range} &  \textbf{Bandwidth} &  \textbf{Clock rate} &  \textbf{Channels} &  \textbf{Cost} 
\\ \hline
\vspace{0.001 in}
B-205 mini &
\vspace{0.001 in}
Spartan-6 XC6SLX150

&
\vspace{0.001 in}

No

&
\vspace{0.001 in}

No
&
\vspace{0.001 in}

Yes
&
\vspace{0.001 in}

70 MHz - 6 GHz
&
\vspace{0.001 in}

56MHz
&
\vspace{0.001 in}

-
&
\vspace{0.001 in}

1x1
&
\vspace{0.001 in}

Low
\\ \hline
\vspace{0.001 in}
B-210
&
\vspace{0.001 in}
Spartan 6 XC6SLX150

&
\vspace{0.001 in}

No

&
\vspace{0.001 in}

No
&
\vspace{0.001 in}

Yes
&
\vspace{0.001 in}

70 Mhz - 6 GHz
&
\vspace{0.001 in}

56 MHz
&
\vspace{0.001 in}

-
&
\vspace{0.001 in}

2x2
&
\vspace{0.001 in}

Low
\\ \hline
\vspace{0.001 in}
X310
&
\vspace{0.001 in}

KINTEX7-410T

&
\vspace{0.001 in}

Yes

&
\vspace{0.001 in}

1GbE/10GbE (SFP+) 
&
\vspace{0.001 in}

No
&
\vspace{0.001 in}

DC - 6 GHz 
&
\vspace{0.001 in}

Up to 160 MHz 
&
\vspace{0.001 in}

Flexible
&
\vspace{0.001 in}

2x2
&
\vspace{0.001 in}

High
\\ \hline
\vspace{0.001 in}
N310 
&
\vspace{0.001 in}

Zynq-7100

&
\vspace{0.001 in}

Yes(not swappable)

&
\vspace{0.001 in}

1GbE/10GbE (SFP+) 
&
\vspace{0.001 in}

No
&
\vspace{0.001 in}

10 MHz - 6 GHz
&
\vspace{0.001 in}

Up to 100 MHz
&
\vspace{0.001 in}

Flexible
&
\vspace{0.001 in}

4x4
&
\vspace{0.001 in}

Very High
\\ \hline
\end{tabular}%
}

\label{tab:HWReq}
\end{table*}



==> include/guidelines.tex <==
Here we can just give some important observations about the building of this testbed to future researchers who wants to build a similar testbed. 
